A methodology to characterize bias and harmful stereotypes in natural language processing in Latin America

Automated decision-making systems, especially those based on natural language processing, are pervasive in our lives. They are not only behind the internet search engines we use daily, but also take more critical roles: selecting candidates for a job, determining suspects of a crime, diagnosing autism and more. Such automated systems make errors, which may be harmful in many ways, be it because of the severity of the consequences (as in health issues) or because of the sheer number of people they affect. When errors made by an automated system affect a population more than others, we call the system \textit{biased}. Most modern natural language technologies are based on artifacts obtained from enormous volumes of text using machine learning, namely language models and word embeddings. Since they are created by applying subsymbolic machine learning, mostly artificial neural networks, they are opaque and practically uninterpretable by direct inspection, thus making it very difficult to audit them. In this paper, we present a methodology that spells out how social scientists, domain experts, and machine learning experts can collaboratively explore biases and harmful stereotypes in word embeddings and large language models. Our methodology is based on the following principles: * focus on the linguistic manifestations of discrimination on word embeddings and language models, not on the mathematical properties of the models * reduce the technical barrier for discrimination experts%, be it social scientists, domain experts or other * characterize through a qualitative exploratory process in addition to a metric-based approach * address mitigation as part of the training process, not as an afterthought

==> Old/annex_case-studies.tex <==
\section{Details on the Case Studies}

\subsection{Case Study 1: Junior Data Scientists}

Group 1:
This group was formed by an Astronomer, an Education Msc, and a PhD in Biology.
They explored low-high resources bias.
\todo{word lists}

Group 2:
This group was formed by an Msc in Business Administration and a Msc in Biology.
They explored origin bias, constructing a Latinamerican and Northamerican spaces.
\todo{word lists}

Group 3:
This group was formed by a Phisics PhD, an Economy Msc and a Electronics Engineer.
They explored socioeconomic bias with regards to sentiments.
\todo{word lists}

Group 4:
This team was formed by a Civil Engineer, an Software Engineer and an Industrial Engineer.
They explored ageism in old and youth spaces.
\todo{word lists}

\subsection{Case Study 2: Social Scientists}

\todo{Amanda: composition of the group}
\todo{Amanda: word lists}

==> Old/assessing.tex <==
\section{Assessing bias} \label{assessing}

Here we present existing tools for biases explorations and situate our proposal with respect to them for word embeddings and large language models (LLMs).

\subsection{Existing frameworks for bias exploration}\label{sec:existing-tools}
%-------------- Paper original-----------------
%%\todo{better integration with the previous and our own design principles}
%%\todo[inline]{Lucía: discuss similarities and differences with existing tools, namely word bias}
%%LUCIANA: Done

%There are tools like WordBias~\cite{Ghai2021} or the Language Interpretability Toolkit \cite{tenney-etal-2020-language} that aim to lower the technical barrier that needs to be climbed to use bias detection and mitigation techniques. These kinds of tools provide implementations of many NLP techniques, and graphical interfaces to avoid having to write code. 

%\cite{DBLP:conf/ijcai/BadillaBP20} is an open source python library called WEFE which is similar to WordBias in that it allows for the exploration of biases different to race and gender and in different languages. One of the focuses of WEFE is the comparison of different automatic metrics for biases measurement and mitigation, however, in order to use this library python programming skills are needed as it doesn't provide a graphical interface.

%None of these frameworks were designed with the goal of being usable by social scientists or people without technical and programming skills in general. WordBias is designed for exploring many different kind of biases, however, it %assumes that languages are non-gendered languages so it is not applicable to Spanish and  has a complex graphical interface not suited for iterative definition of word lists. The Language Interpretability Tool includes (among many other capabilities) interactive visualizations, integrated fairness and explicability metrics, counterfactual analysis, etc. These tools require extensive Natural Language Processing understanding from the user. In general, most of the toolkits, frameworks and libraries providing functionalities to assess model behaviour with respect to biases are confuse and opaque even for developers with extensive technical knowledge \cite{10.1145/3411764.3445604}. 
%-----------------------------------------

%-------Propuesta Mariela-----------------
\todo[inline]{Mariela: ¿Agrego aquellas librerías que permiten evaluar bias pero que requieren de conocimientos de Python?}
\todo[inline]{Luciana: No sé exactamente a qué te referís, yo agregué abajo WEFE porque se lo mencionaba sin introducirlo.}

%LB: I comment this paragraph because I think it is unprecise and repetitive wrt other sections. This is better described in other sections. 
%\textcolor{violet}{The embedding bias analysis requires comparisons and inspection of large volumes of text. To decide if a word (or a sentence) is biased the main study consists in comparing the similarity of the word (or sentence) with the list of words assigned to each of the categories. In embeddings, each word is represented by a vector, and analyzing similarities between words consists in calculating the similarities between the words' vector representation. Generally, these methodologies are implemented in a framework so that researchers can focus on the bias analysis and avoid having to write code. }

Multiple frameworks were developed in the last years for bias analysis. Most of them require mastery of machine learning methods and programming knowledge. Others have a graphic interface and may reach a larger audience. %that facilitates the analysis, especially for researchers without technical skills. 
%Although the possibility of accessing a graphical interface is one of the most obvious barriers to bias analysis in embeddings, other aspects such as the options present in the interfaces, the types of bias, 
%are decisive in being able to create interdisciplinary bias analysis with diverse perspectives corresponding to experts from different study areas  None of these frameworks were designed with the goal of being usable by social scientists or people without technical and programming skills in general. 
However, having a graphical interface is certainly not enough to guarantee an analysis without relying on researchers with machine learning skills. In order to create interdisciplinary bias analysis, it will be relevant that the analysis options present in the graphical interfaces, and data visualizations and manipulation are oriented toward a non-technical audience. In the following, we give a brief description of some of the frameworks with graphical interfaces available for bias analysis of embeddings or language models.

\textcolor{violet}{WordBias \cite{Ghai2021} is a framework that aims to analyze embeddings biases by defining lists of words. In WordBias, new variables and lists of words may be defined. This framework allows the analysis of intersectional bias. The bias evaluation is done by a score based on cosine distance between vectors and does not allow the incorporation of other metrics. Until October 2022, this framework is only available to analyze the word2vec embedding, without having the possibility to introduce other embeddings or models.} 

\textcolor{violet}{VERB \cite{Rathore2021} enables bias analysis in embeddings altohough it is focused on bias mitigation strategies. This framework is orientated to researchers with algorithmic, linear algebra and metrics skills.}

\textcolor{violet}{What-if tool \cite{Wexler2019} is a framework that enables the bias analysis corresponding to a diverse kind of data. Although it is not focused on text data it allows this type of input. What-if tool offers multiple kinds of analysis, visualization, and evaluation of fairness through different metrics. To use this framework researchers with technical skills will be required to access the graphic interface due to is through Jupyter/ Colab Notebooks, Google Cloud, or Tensorboard, and, also, because multiple analysis options require some machine learning knowledge (e.g, selections between AUC, L1, L2 metrics). Own models can be evaluated but since it is not text-specific, it is not clear how the evaluation of words or sentences will be. This tool allows the evaluation of fairness through different metrics.}

\textcolor{violet}{The Language Interpretability Tool (LIT) \cite{Tenney2020} is an open-source platform for visualization and analysis of NLP models. It was designed mainly to understand the models' predictions, to explore in which examples the model underperforms, and to investigate the consistency behavior of the models by analyzing controlled changes in data points. LIT allows users to add new datapoints on the fly,  to compare two models or data points, and provides local explanations and aggregated analysis. However, this tool requires extensive Natural Language Processing understanding from the user.}

\cite{DBLP:conf/ijcai/BadillaBP20} is an open source Python library called WEFE which is similar to WordBias in that it allows for the exploration of biases different to race and gender and in different languages. One of the focuses of WEFE is the comparison of different automatic metrics for biases measurement and mitigation, however, in order to use this library python programming skills are needed as it doesn't provide a graphical interface.

%LIT provides aggregate analysis, it allows users to test local hypotheses and validate them on the dataset, to add new data points on the fly,  comparisons for two models or two data points and local explanations. However, this tool require extensive Natural Language Processing understanding from the user.

%------Fin propuesta Mariela

Our methodology builds on the Responsibly~\cite{responsibly} 
%toolkit based on~\cite{10.5555/3157382.3157584} as we explained in the previous section. We selected Responsibly because it focuses on exploration with the most simple metric of bias (direction projection)
%\todo{Pondría que hace direction projection, al menos una intuición} 
%rather than on the comparison of different automatic biases measurements as WEFE does. %Among other things, this toolkit provides a high level implementation of "hard debias", "soft debias", WEAT, and other Word Embedding bias detection and mitigation techniques. 
Responsibly is based on previous work by \citet{10.5555/3157382.3157584} which establishes an approach to the problem that is intuitive as we explained in the previous section and illustrated in Figure~\ref{fig:english-spanish}.%, but at the same time establishes some of the oversimplifications that have been carried on in most of the subsequent work. 

%LB: This is explained in the previous section
%This technique is presented for the English language and gender and racial biases but it can be applied to any bias that can be modeled as binary in languages that do not have grammatical gender. %Languages other than English have different properties that are rarely dealt with when processing English, like grammatical gender. 

%LB: This is better described in the previous section already
%However, in order to be able to use the Responsibly toolkit a person should have python programming skills, understanding on word embeddings, natural language processing and bias in word embeddings. Moreover, this person, unless they are working in an interdisciplinary team, should also have expertise on which biases present in word embeddings are relevant to the problem and could affect downstream applications. In our project, we propose to integrate the functionalities provided by Responsibly in a tool that facilitates the engagement of people without technical skills in the process of bias assessment.






%\todo{finish with a compact summary of what we think is valuable in contrast with what the focus has been put on, a summary that will be taken in the beginning of the following section. The first paragraph in the following section will be something like this: "As follows from the discussion of relevant work, the design principles of this methodology are: reduction of the technical barrier, focus on exploration and characterization of bias (instead of focus on a compact, opaque, metric-based diagnostic), with word lists as a dynamic, interactive way to elicit, shape, express expert knowledge (instead of taking lists as given by other papers, even if these are papers from social scientists), attention to linguistic and cultural aspects that may bias word lists (instead of just translating word lists from another language or taking professions as neutral). "}

\subsection{Assessing bias in word embeddings}

%LB: repeated
%Fortunately, given the importance that word embeddings have in language technologies, and the impact that biases may have, in the last years we have seen the emergence of a wide range of tools and techniques to assess bias in word embeddings and language models. 

Our core methodology to assess biases in word embeddings consists of three main parts (illustrated in Figure~\ref{fig:english-spanish} described in the previous section). The three parts are the following. 

\begin{enumerate}
    \item Defining a \textbf{bias space}, usually binary, delimited by pairs of two opposed extremes, as in \textit{male -- female}, \textit{young -- old} or \textit{high -- low}. Each of the extremes of the bias space is characterized by a list of words, shown at the top of the diagrams in Figure~\ref{fig:english-spanish}.
    \item Assessing the behaviour of \textbf{words of interest in this bias space}, finding how close they are to each of the extremes of the bias space. This assessment shows whether a given word is more strongly associated to any of the two extremes of bias, and how strong that association is. In Figure~\ref{fig:english-spanish} it can be seen that the word "\textit{nurse}" is more strongly associated to the "\textit{female}" extreme of the bias space, while the word "\textit{leader}" is more strongly associated with the "\textit{male}" extreme. 
    \item Acting on the conclusions of the assessment. The actions to be taken vary enormously across approaches, as will be seen in the next section, but all of them are targeted to \textbf{mitigate} the strength of the detected bias in the word embedding.
\end{enumerate}

This form of bias assessment characterizes words in isolation. However, some aspects of the meaning of utterances depend on the combination, in the co-occurrence of words. LLMs represent contextual meaning. \todo{develop}

\subsection{Assessing bias in LLMs}

As exemplified in Section \ref{sec:llms}, LLMs represent contextual meaning. This meaning cannot be analyzed in the analytical fashion that we have seen for word embeddings. However, it can be queried in terms of preferences, that is, how probable it is that a LLM will produce a given sentence. Thus, we can assess the tendency of a given LLM to produce racist, sexist language or, in fact, language that invisibilizes or reinforces any given stereotype, as long as it can be represented in contrasting sequences of words.

A sound methodology to explore biases in LLMs is proposed by \citet{zhao-etal-2019-gender,sedoc-ungar-2019-role}\todo{include also french crows pairs, check all relevant refs are included}. %Contextual embeddings exhibit similar biases to those in word embeddings when trained on the same data~\cite{zhou-etal-2022-sense}. exploration of contextual embeddings
It consists on manually producing contrasting pairs of utterances that represent two versions of a scene, one that reinforces a stereotype and the other contrasting with the stereotype (what they call \textit{antistereotype}). Then, the LLM is queried to assess whether it has more preference for one or the other, and how much. This allows to assess how probable it is that the LLM will produce language reinforcing the stereotype, that is, how biased it is for or against the encoded stereotype.

Thus, the inspection of LLMs complements that of word embeddings.

==> Old/discussion.tex <==
\section{Discussion and limitations}

modelar extremos donde uno no está lexicalizado, futbol

modelado binario, interseccionalidad

cuando parar de modificar las listas

out of word vocabulary





==> Old/introduction-old.tex <==
\section{Introduction} \label{sec:introduction}

\todo{see alt\_introduction for a suggestion on reorganizing this section}

Lexical methods for bias measurement use seed lexicons, but there are no previous user studies on trying to involve social scientists in the selection of such hand-curated lexicons. 

\citet{antoniak-mimno-2021-bad} argue that “While there is a wide range of bias measurement methods, every one of them relies on lexicons of seed terms to specify stereotypes or dimensions of interest. But the rationale for choosing specific seeds is often unclear; sometimes seeds are crowd-sourced, sometimes hand-selected by researchers, and sometimes drawn from prior work in the social sciences”. To make matters worse, these lexicons of seed terms encode biases of their creators that are reproduced by other machine learning practitioners using the same seeds without scrutiny. For example, \citet{10.1145/2858036.2858535} include the crowd sourced words `dominate', `intimidating' and `overpowering' in their definition of the concept `masculine', and `cleavage', `fuchsia' and `skinny' in their definition of the concept `female'. 

Machine learning models and data-driven systems are increasingly being used to support decision-making processes. Such processes may involve fundamental rights, thus it is important that models can be inspected and judged by a wider range of actors, many of which do not have technical expertise. The objective of this project is to adapt and facilitate a tool for the detection, diagnosis, prevention of bias in natural language processing applications, focused on the specific needs of the Latin American region. In Latin America, we need domain experts to be able to carry out these analyses with autonomy, not relying on an interdisciplinary team or on training, both are usually not at hand. In particular, this tool involves defining the seed lexicons in an interative way and providing support for adapting the lexicons through an exploratory process. 

Dealing with biases, and in general deploying fairness within Artificial Intelligence requires an adequate understanding of  complex sociological constructs, often involving phenomena that are not well understood, let alone systematized or formalized. Formalizing such constructs for computational treatment is challenging, and requires the involvement of experts: sociologists, linguists, physicians, psychologists among others. However, much of the development to deploy fairness, like fairness metrics and frameworks, are based on nuanced technical instruments that hinder understanding and involvement of individuals without extensive technical education including programming skills. This is the case of techniques for diagnosing and mitigating bias in word embeddings.

Word embeddings are widely used natural language processing artifacts that represent the meaning of words fully automatically, based on their usage in large amounts of text. The gist of word embeddings consists in representing word meanings as similar if they cooccur with similar words in large volumes of text. This is why it is necessary to have large volumes of text to train word embeddings.  

%Most Natural Language Processing systems use word representations generated by neural networks, such as word embeddings [11]. These representations are mainly used in downstream tasks such as translation, style correction, or text auto complete [18].
%It has been noted that word embeddings incorpore bias and prejudice such as associating certain professions to a gender [17]. These biases contribute to the invisibilization of minorities and stereotyping, but we are facing a shortage of methods of detection and mitigation, especially for languages apart from english [cita lit review?].

These artifacts are deployed in applications such as text auto-completion or automatic translation, and have been shown to improve the performance of virtually any natural language processing task they have been applied to. The problem is that word embeddings are obtained from large volumes of texts that have underlying biases and prejudices. Such biases are carried into the representation which are thus transferred to applications. But since these embeddings are complex and opaque artifacts, it is very difficult to detect the biases. In spite of that opacity, readily available pre-trained embeddings are widely used in socio-productive solutions, like rapid technological solutions to scale and speed up  response to the COVID19 pandemic.

With this project, we will provide tools and techniques to analyze word embedding biases and mitigate them, with a special focus on Argentinean and Latin American Spanish. We will pay special attention to gender biases, against migrants, aporophobia, ableism, and the marginalization of historically disadvantaged communities. This context differs significantly from that of similar studies and lines of work in countries of the global north.

The tools developed within this project will make it easier for people without prior technical knowledge to use technologies developed in academic institutions in the global north. In this way, we will seek to minimize technological barriers, so that regional experts in fields such as sociology, social work, economics, communication, referents of different communities, education, etc., can impact these central technological artifacts of Artificial Intelligence with their specific knowledge.

This paper is organized as follows. Section 2 presents previous work in the area of bias diagnostics and mitigation in word embeddings and also arguments why this technology underlies and shapes the behavior of current natural language technologies. Section 3 explains the rationale for our approach and how it puts the power to diagnose and mitigate biases in the hands of people with the knowledge and the societal roles to have an impact on current technologies. Section 4 presents the prototype we plan to implement to achieve our goal. Section 5 describes two sets of case studies in which we test a mock up of our prototype with our guidance with two groups of subjects. The first group are data scientists with different expertise backgrounds but at least a 350 hours of training and education in data science (including the development and evaluation of machine learning models). The second group are social scientists with no previous training in programming or technical aspects of machine learning. Section 6 integrates a look at the public policy and regulatory aspects associated with different forms of discrimination and the emergence of bias in word embedding systems.  Although there are currently numerous initiatives on artificial intelligence regulations, in this paper we will deal exclusively with those that have to do with discrimination of disadvantaged groups and we will make a brief mention of the challenges in terms of intellectual property.  Section 7 includes our conclusions and next steps.  


==> Old/methodology.tex <==
\section{Methodology to lower barriers for bias exploration} \label{sec:methodology}

In this Section we present our methodology to engage experts without technical skills in the assessment of biases in word embeddings. As follows from the discussion of relevant work, the design principles of this methodology are: reduction of the technical barrier, focus on exploration and characterization of bias, %(instead of focus on a compact, opaque, metric-based diagnostic), 
with word lists as a dynamic, interactive way to elicit, shape, express expert knowledge, %(instead of taking lists as given by other papers, even if these are papers from social scientists), 
attention to linguistic and cultural aspects that may bias word lists. %(instead of just translating word lists from another language or taking professions as neutral). 

\subsection{Reducing the technical barrier}

This methodology has been delivered by composing with the building blocks from the Responsibly library and interactive notebook \citet{responsibly}. Our current approach to involve experts in this task is through their use of a simplified version of this interactive colab notebook, as an intermediate phase before a full-fledged prototype can be developed. This intermediate phase has been useful to observe how different kinds of users ***

In the first place, we have removed as many technicalities as possible from the explanation of the science behind word embeddings, the representation of bias as a direction in the embedding space, the calculation of bias and the ***. We basically explain word embeddings as an artifact where words are represented by their contexts of occurrence


\todo[inline]{the following paragraph originally in motivation, but I think it is better suited here}
the complexity of the task in constructs that are intuitive for domain experts to pour their knowledge, formulate their hypotheses and understand the empirical data. Conversely, we try to keep the technical complexity of the approach to a bare minimum.

\subsection{Dynamic exploration of the bias space}

currently an interactive colab notebook (w screenshots)

\subsection{Linguistic, statistic and cultural aspects of words}

Since words are the keystone, 

Bad seeds say there are biases in word lists. We cannot be rid of bias but we can make it explicit, document it, and make it part of the characterization.

Special care must be taken to not directly apply the approach for English to any other language, because other languages can have their own linguistic differences
    
it is language independent but language particularities need to be taken into account because if not the particularities will mess with the assumptions of the methodology. But most of these particularities can be accommodated involving specialized linguistic knowledge. A good example is gender and pro-drop.

\todo[inline]{the following paragraph originally in motivation, but I think it is better suited here}
In this paper we show how gender bias in languages with morphologically marked grammatical gender can be adequately characterized with a simple approach to bias, namely \citet{Bolukbasi2016ManIT}. That is, the complexity of modelling morphological gender with an additional dimension can be replaced by putting domain knowledge into the design of word lists. We show the very positive impact of applying linguistic reasoning to include different words to model the gender dimension or to explore different aspects of bias in the dimension.

Summary of the methodology:

\begin{enumerate}
    \item explain without technicalities the fundamental concepts of the approach: 
    \begin{itemize}
        \item word embeddings approximate the meaning of words as a summary of their contexts, so that words that share a high proportion of contexts are close
        \item we can represent a certain bias as a binary continuum of meaning, by defining words that are in its two extremes of this continuum
        \item we can see how any given word is positioned in this continuum of bias
    \end{itemize}
    \item represent a bias of interest, putting an effort in identifying linguistic and cultural issues that may affect the words chosen to represent the extremes of bias, and document such issues as explicitly as possible.
    \begin{itemize}
        \item frequency of the words **
        \item polysemy ***
        \item different distribution of words in the two extremes with respect to the meaning of interest, for example words in slang in one of the extremes and very technical words in the other, for example, representing age bias with the sets of words: \textit{elder}, \textit{aged}, \textit{venerable} in one extreme and \textit{kiddo}, \textit{pup}, \textit{lass} in the other.
        \item 
    \end{itemize}
    \item put the emphasis on exploration, comparing different effects. Experts can formulate hypotheses as to how sets of words will be positioned in a given continuum of bias, for example:
    \begin{itemize}
        \item sets of words that we would expect to be at the same distance from the two extremes of bias
        \item the effect of different words on the definition of the bias space of 
        \item intersectionality
    \end{itemize}
    \item diagnosing bias by describing the 
    \item mitigating bias by curating the corpus
\end{enumerate}

*** to case studies:


Limitations: multiword expressions

Social scientists and linguists wanted to know more about how word embeddings were constructed and how "context" was defined. They had a keen interest in 

Then

*** to following steps in the prototype:

intersectionality by expressing intersections in the extremes

==> Old/motivation.tex <==
\section{Motivation} \label{sec:motivation}

From an academic perspective, the complexity of bias is well-acknowledged [REF MISSING]. There is a consensus [REF MISSING] that what we call bias are the observable (if subtly) phenomena from underlying causes deeply rooted in social, cultural, economic dynamics. Such complexity falls well beyond the social science capabilities of most of the computer scientists currently working on bias in artificial intelligence artifacts. Most of the effort of ongoing research and innovation wrt bias is concerned with technical issues. In truth, these technical lines of work are aimed to develop and consolidate tools and techniques more adequate to deal with the complex questions than to build a solid, reliable basis for them. However, such developments have typically resulted in more and more technical complexity, which hinders the engagement of domain experts. Such experts could provide precisely the understanding of the underlying causes that computer scientists lack, and which could help in a more adequate model of the relevant issues. In this section we illustrate BLA, we motivate our approach and C. 

For example, in modelling gender bias, the first approaches were developed for English. English is a language where morphological marking of grammatical gender is residual, observable in the form of very few words, mostly personal pronouns and some lexicalizations like “actress - actor”. Some of the assumptions underlying this approach seemed inadequate to model languages where a big number of words have a morphological mark of grammatical gender, like Spanish or German, where most nouns or adjectives are required to express a morphological mark for different grammatical genders. The proposal from the computer science community working on bias was a more complex geometric approach, with a dimension modelling semantic gender and another dimension modelling morphological gender. Such approach is more difficult to understand for people without a computer science background, which is usually the case for social domain experts that could provide insight on the underlying causes of the observable phenomena.

In this work we have explored the effects of putting the complexity of the task in constructs that are intuitive for domain experts to pour their knowledge, formulate their hypotheses and understand the empirical data. Conversely, we try to keep the technical complexity of the approach to a bare minimum.

%Aligned with similar work, we show that bias in word embeddings can be satisfactorily explored, characterized and mitigated by putting most of the effort into word lists, instead of tools to manipulate vectors, spaces or complex mathematical relations between abstract mathematical concepts, far removed from the understanding of the underlying issues that cause bias.

In this paper we show how gender bias in languages with morphologically marked grammatical gender can be adequately characterized with a simple approach to bias, namely \citet{Bolukbasi2016ManIT}. That is, the complexity of modelling morphological gender with an additional dimension can be replaced by putting domain knowledge into the design of word lists. We show the very positive impact of applying linguistic reasoning to include different words to model the gender dimension or to explore different aspects of bias in the dimension.

Moreover, we also show that reducing the technical complexity of the tool and explanations to the minimum fosters engagement by domain experts. Providing intuitive tools like word lists, instead of barriers like vectors, allows them to formalize their understanding of the problem, casting relevant concepts and patterns into those tools, formulating hypotheses in those terms and interpreting the data. Such engagement is useful in different moments in the software lifecycle: error analysis, framing of the problem, curation of the dataset and the artifacts obtained therefrom...

In the next section we present our methodology and in Section~\ref{sec:first-tool} we present its intended use cases. 


This is precisely the kind of involvement that can enrich approaches to bias originated in the computer science community with the necessary domain knowledge to adequately model the problems of interest. The reduction in technical complexity is not to justify an over-simplification of the problems, as is often the case under time constraints. On the contrary, with this approach we are advocating that resources should be devoted to where complexity is most needed, that is, in the understanding and modelling of the causes, not on the creation of different artifacts to manipulate data.



==> Old/policy.tex <==
\section{Potential impacts on policy} \label{sec:policy}

Artificial intelligence systems are not new, they have decades of work, progress and setbacks. However, in these first two decades of the 21st century, implementations of automated decision-making systems have proliferated in various fields of social activity. Many decisions that affect people's lives are made directly by automatic systems, without even the slightest human supervision. Algorithms have gained importance in public life, taking decisive roles in the lives of many people. Approving a loan, obtaining a school vacancy, analyzing tax profiles, filtering resumes for a job, granting or denying access to visas, and many other decisions are mediated by automated systems. Research in the social sciences today needs to deal with algorithms as a key component of social organization and balance of power. 

%***but it is not easy because of lack of technical skills and 

The transparency of these mechanisms is one of the challenges faced by those who make public policy decisions, especially to assess whether these automated decision-making processes are compliant with regulations and legal standards. However, the declared objective of transparency does not seem to be enough to solve the problems derived from the potential associated problems. It is essential to think of strategies that allow these systems to function responsibly and in accordance with the law.  In this work we analyze only some aspects associated with the general regulatory framework. This clipping is directly related to the object of this project and the tools in use for it.  

\subsection{Human Rights and biases in NLP}

The Universal Declaration of Human Rights approved in 1948 establishes the general normative framework saying that "All human beings are born free and equal in dignity and rights and, endowed as they are with reason and conscience, they must behave fraternally towards one another" and continues "Everyone is entitled to the rights and freedoms set forth in this Declaration, without distinction of any kind as to race, color, sex, language, religion, political or other opinion, national or social origin, property, birth or other status."

However, human society is far from fulfilling this vision of those who promoted and promote equality and justice as fundamental rights. Discrimination based on ethnicity, color, gender, language, religion, opinion, economic position and diversity of abilities continue to be the order of the day despite the legal frameworks established for its eradication.  

In Argentina, since 1994, the "American Declaration of the Rights and Duties of Man; the Universal Declaration of Human Rights; the American Convention on Human Rights; the International Covenant on Economic, Social, and Cultural Rights; the International Covenant on Human Rights have constitutional status." Civil and Political Rights and its Optional Protocol, the Convention on the Prevention and Punishment of the Crime of Genocide, the International Convention on the Elimination of All Forms of Racial Discrimination, the Convention on the Elimination of All Forms of Discrimination Against Women; the Convention Against Torture and Other Cruel, Inhuman or Degrading Treatment or Punishment; the Convention on the Rights of the Child; in the conditions of their validity, they have constitutional hierarchy, do not repeal any article of the first part of this Constitution and must be understood as complementary of the rights and guarantees recognized by it. They can only be denounced, where appropriate, by the National Executive Power, prior approval of two thirds of all the members of each Chamber. 

That same constitutional framework is shared by the countries of all of Latin America, the region from which we carried out this investigation. It is this framework of Human Rights that establishes the normative base that later derives in specific regulations on each of the fields addressed in this field. However, we understand that specific legislation is not necessary for the uses and applications of automated decision-making systems, but rather the possibility of applying the current regulatory and legal frameworks, with the consequent fulfillment of guarantees and rights established with the highest legal rigor  

\subsection{Ethics and regulation}

Various international organizations, including UNESCO, have initiated processes for the creation of ethical frameworks for the development, adoption and implementation of artificial intelligence technologies in public life. However, these ethical safeguards that must be disseminated and adopted by all interested parties, must have a strong regulation. 

UNESCO highlights various edges from which it is necessary to work, starting with an express and explicit prohibition of any system of social markers and mass surveillance. The use of AI systems for qualifying people and for mass surveillance should be strictly prohibited. Faced with this problem, the States have the duty to establish accountability mechanisms that establish the responsibility of the people in charge. 

The protection of personal data, together with the protection of privacy, is another of the nodal axes of regulatory work where the ethical issue is severely limited. Strong regulations, civil and criminal liability systems, as well as data processing compliance mechanisms, are key, all accompanied by enforcement authorities that meet the basic conditions to have a positive impact on the defense of Human Rights. 

Of course, all technology must have, before it is put into operation, various metrics and tools for an appropriate impact assessment. This impact must consider not only the life trajectory of the people affected, but also the impact that they have on the environment and care for the planet, with particular attention to energy consumption, the impact of emissions and the climate crisis and the impact on ecosystems. 

\subsection{Aspects linked to intellectual property}

Intellectual property regulatory systems go through regulations on artificial intelligence systems from the outset on at least three levels: the regulation of software development, the regulation of data sources for training and the regulation of the results of the AI application. 

Intellectual property systems have regulated the development of the software industry for several decades. From the integration of computer programs to the world of Copyright in the US in the 1970s to its integration into the Agreements on Intellectual Property Aspects Applied to Trade of the World Trade Organization in 1995, there is a global regulatory harmonization in the matter. %However, in some states patents on mathematical algorithms are also recognized (Diamond v. Diehr - US1980).

Training data sources pose a major challenge, since databases also have copyright regulations. Added to this is the diversity of training sources. In natural language processing, the use of texts for training can pose a problem due to the unauthorized use of certain texts from specific areas, since they are regulated under copyright and copyright regulations. This is one of the reasons why texts published in the public domain (such as court rulings, legislation) or under conditions of free use and distribution (such as Wikipedia) are widely used, with the potential biases and thematic limitations that this implies. 

Finally, despite the fact that the recommendations of UNESCO emphasize the idea that legal personality should not be granted to AI systems, there are not a few that have already initiated legal and legal actions aimed at achieving the conformation of what is provisionally called "artificial author" to attribute ownership to products developed by AIs. This debate may seem abstract, however it has an impact both in terms of civil liability and in economic matters, since advancing in this line supposes a novel form of private appropriation of an intangible asset whose creation does not depend on an individual author but on a multiplicity of processes.



%Abajo está la versión en español original de Bea

%Los sistemas de inteligencia artificial no son nuevos, tienen décadas de trabajo, avances y retrocesos. Sin embargo, en estas primeras dos décadas del siglo XXI han proliferado las implementaciones de sistemas automatizados de toma de decisiones en diversos campos del quehacer social. Muchas decisiones que afectan la vida de las personas son tomadas directa y exclusivamente por sistemas de cómputo. Los algoritmos han ganado visibilidad y preminencia en la vida pública y se han vuelto protagonistas de la vida de muchas personas. Aprobar un crédito, obtener una beca de investigación, analizar perfiles impositivos, realizar una preselección de curriculumns para un empleo, otorgar o negar acceso a visas y muchas otras decisiones están mediadas por sistemas automatizados. La investigación en ciencias sociales hoy no puede permanecer ajena a esta realidad. 

%La transparencia de estos mecanismos es uno de los desafíos a los que se enfrentan quienes toman decisiones de políticas públicas, especialmente para evaluar cómo se aplican o no los estándares legales en estos procesos de toma de decisiones automatizadas. Sin embargo, el objetivo declarado de transparencia no parece ser suficiente para solucionar los problemas derivados de los potenciales problemas asociados. Es indispensable pensar estrategias que permitan hacer que estos sistemas funcionen de manera responsable y ajustados a derecho.  

%En el marco de este trabajo analizamos sólo algunos aspectos asociados al marco regulatorio general. Este recorte tiene directa relación con el objeto de este proyecto y las herramientas en uso para el mismo.  

%Un marco de Derechos Humanos para la identificación y mitigación de sesgos en aplicaciónes de procesamiento de lenguaje natural 

%La Declaración Universal de los Derechos Humanos establecida en 1948 fija el marco normativo general en el que se establece como base que  "Todos los seres humanos nacen libres e iguales en dignidad y derechos y, dotados como están de razón y conciencia, deben comportarse fraternalmente los unos con los otros." y continúa " Toda persona tiene los derechos y libertades proclamados en esta Declaración, sin distinción alguna de raza, color, sexo, idioma, religión, opinión política o de cualquier otra índole, origen nacional o social, posición económica, nacimiento o cualquier otra condición."

%Sin embargo, la sociedad humana está lejos de cumplir con esta visión de quienes impulsaron y quienes promueven la igualdad y la justicia como derechos fundamentales. La discriminación por étnia, color, género, idioma, religión, opinión, posición económica y diversidad de capacidades siguen a la orden del día pese a los marcos legales establecidos para su erradicación.  

%En Argentina, desde 1994 tienen rango constitucional "la Declaración Americana de los Derechos y Deberes del Hombre; la Declaración Universal de Derechos Humanos; la Convención Americana sobre Derechos Humanos; el Pacto Internacional de Derechos Económicos, Sociales y Culturales; el Pacto Internacional de Derechos Civiles y Políticos y su Protocolo Facultativo; la Convención Sobre la Prevención y la Sanción del Delito de Genocidio; la Convención Internacional sobre la Eliminación de Todas las Formas de Discriminación Racial; la Convención Sobre la Eliminación de Todas las Formas de Discriminación Contra la Mujer; la Convención Contra la Tortura y Otros Tratos o Penas Crueles, Inhumanos o Degradantes; la Convención Sobre los Derechos del Niño; en las condiciones de su vigencia, tienen jerarquía constitucional, no derogan artículo alguno de la primera parte de esta Constitución y deben entenderse complementarios de los derechos y garantías por ella reconocidos. Sólo podrán ser denunciados, en su caso, por el Poder Ejecutivo Nacional, previa aprobación de las dos terceras partes de la totalidad de los miembros de cada Cámara. "

%Ese mismo marco constitucional comparten los países de toda América Latina, región desde la cual realizamos la presente investigación.  Es ese marco de Derechos Humanos el que fija la base normativa que deriva luego en regulaciones específicas sobre cada uno de los campos abordados en este campo. Sin embargo, entendemos que no hace falta una legislación específica para los usos y aplicaciones de sistemas automatizados de toma de decisiones, sino la posibilidad de aplicar los marcos regulatorios y legales vigentes, con el consiguiente cumplimiento de garantías y derechos establecidos con el más alto rigor legal.  

%Ética y regulación

%Diversos organismos internacionales, entre ellos la UNESCO, han iniciado procesos para la conformación de marcos éticos de desarrollo, adopción e implementación de tecnologías de inteligencia artificial en la vida pública. 

%Sin embargo, esos resguardos éticos que deben ser difundidos y adoptados por todas las partes interesadas, deben tener un correlato regulatorio fuerte. 

%UNESCO destaca diversas aristas desde las cuales es menester trabajar, empezando por una prohibición expresa y explícita de cualquier sistema de marcador social y vigilancia masiva. Se debe prohibir taxativamente el uso de sistemas de IA para calificación de las personas y parala vigilancia masiva. Frente a esta problemática, los Estados tienen el deber de establecer mecanismos de rendición de cuentas que fijen la responsabilidad en las personas a cargo. 

%La protección de datos personales, junto con la protección de la privacidad, es otro de los ejes nodales de trabajo regulatorio donde la cuestión ética se ve severamente limitada. Regulaciones fuertes, sistemas de responsabilidad civil y penal así como mecanismos de observancia sobre el procesamiento de datos es clave, todo esto acompañado de autoridades de aplicación que reúnan las condiciones básicas para incidir positivamente en la defensa de Derechos Humanos. 

%Por supuesto, toda tecnología debe contar, antes de su puesta en funcionamiento, con métricas y herramientas diversas para una apropiada evaluación de impacto. Ese impacto debe contemplar no sólo la trayectoria vital de las personas afectadas, sino también el impacto que las mismas tengan en el medioambiente y el cuidado del planeta, con particular atención en el consumo de energías, el impacto de las emisiones y la crisis climática y el impacto en los ecosistemas. 

%Aspectos vinculados a propiedad intelectual 

%Los sistemas regulatorios de la propiedad intelectual atraviesan desde el origen las regulaciones sobre los sistemas de inteligencia artificial en al menos tres niveles: la regulación de los desarrollos de software, la regulación de las fuentes de datos para entrenamiento y la regulación de los resultados de la aplicación de IA. 

%Los sistemas de propiedad intelectual regulan el desarrollo de la industria de software desde hace varias décadas. Desde la integración de los programas de cómputo al mundo del Copyright en los EEUU en la década del 70 hasta su integración en los Acuerdos sobre Aspectos de Propiedad Intelectual aplicados al Comercio (ADPIC) de la Organización Mundial de Comercio en 1995 existe una armonización regulatoria global en la materia. Sin embargo, en algunos Estados se reconocen además patentes sobre algoritmos matemáticos (Diamond v. Diehr - US1980).

% Las fuentes de datos para entrenamiento suponen un desafío mayúsculo, toda vez que las bases de datos también tienen regulaciones de copyright. A esto se suma la diversidad de fuentes de entrenamiento. En procesamiento de lenguaje natural, el uso de textos para entrenamiento puede suponer un problema por el uso no autorizado de ciertos textos de áreas específicas, ya qua que los mismos se encuentran regulados bajo las normas de derecho de autor y copyright. Esta es una de las razones por las cuales se usan de manera masiva textos publicados en dominio público (como sentencias judiciales, legislaciones) o bajo condiciones de libre uso y distribución (como Wikipedia) con los potenciales sesgos y limitaciones temáticas que esto implica. 

%Finalmente, pese a que las recomendaciones de UNESCO enfatizan en la idea de que no se debe otorgar personalidad jurídica a los sistemas de IA, no son pocos los que ya han iniciado acciones jurídicas y legales tendientes a lograr la conformación de lo que se denomina provisoriamente "autor artificial" para atribuir titularidad a los productos desarrollados por IAs.  Este debate puede parecer abstracto, sin embargo supone impacto tanto en materia de responsabilidad civil como en materia económica, ya que avanzar en esta línea supone una forma novedosa de apropiación privada de un bien intangible cuya creación no depende de un autor individual sino de una multiplicidad de procesos. 


==> Old/proposed_narrative.tex <==
\todo[inline]{proposal for a narrative structure of the paper}

\begin{enumerate}
    \item ? FAIR intro what is bias? non-random distribution of error, most interestingly when it damages people, most interestingly when those people are marginalized communities
    \item ? FAIR intro scope: nlp
    \item ? FAIR intro what is bias in nlp
    \item what is ethical audit, why it is important and which kind of problems it addresses in nlp
    \item MARIE + LAURA NEW general structure of audits in ml approaches: training data (descriptive: prevalences of features and classes), its recollection process and its curation (data sheets for datasets), predictive models (distribution of error) (not framing or deployment context, which is ethics oversight, we only do algorithmic audits)
    \item ? FAIR intro adding LMs which artifacts (within the predictive models) are most important to diagnose: those more pervasive and more opaque: word embeddings and language models. We focus on those and not algorithms, including rules
    \item ? NEW How to decide what features and tools are necessary to carry out a proper, thorough characterization of bias, satisfactory to all involved parties (because bias is always a community thing, not a well-defined, standalone, objective, universal concept). First, we took a stance that we wanted domain experts to have a more central role in the process, then we assumed they did not have the technical skills, then we developed a first approach and worked together with diverse experts to find out about their needs to carry out the task. 
    \item ? Obtaining the input, but heavily restructured, from FAIR section use cases. Applying this process, we found these to be important features and tools to characterize biases in nlp artifacts (word embeddings and language models):
    \begin{itemize}
        \item less focus on metrics, more focus on representation of domain knowledge (word lists, sentence pairs)
        \item integration of tools to aid the decisions as to how to configure knowledge resources, e.g. word frequencies, contexts of occurrence, vicinity in the embedding
        \item more flexibility and expressivity in how these knowledge resources can capture phenomena and assess their representation in the model, that is, dealing with ambiguity of words, dealing with non-binary, possibly unmarked meanings (indígena vs. no indígena), complex, composable meanings (intersectionality), multiword expressions, assessment of generative behaviour in general 
    \end{itemize}
    \item [MARIE] [SECTION] considering these needs, what are the options? ( \url{https://docs.google.com/document/d/106yLR8cWNSxL0d1fFea9SybtCgq8R-mVNw_6dRNKMlo/edit originally section 3})
    \begin{itemize}
        \item academic proposals to deal with bias: 
        \begin{itemize}
            \item they pay more attention to metrics and mitigation than to knowledge resources, even if they have known for a long time (bad seeds) that knowledge resources are more determinant,
            \item they address complexity in the phenomena by creating technically more complex approaches
            \item they only deal with few, very specific biases (gender, race), that are heavily lexicalized, thus more shallow than most biases
        \end{itemize}
        \item frameworks: they try to be more friendly but still they require a huge amount of technical skills and knowledge to run and interpret results, and do not provide expressivity to address specific complexities of language, like ambiguity.
    \end{itemize}
    \item [?] [SECTION, FAIR section 5, mostly 5.1] our proposal
    
\end{enumerate}


==> Old/prototype.tex <==
\section{A prototype for bias assessment in word embeddings and large language models} \ref{sec:prototype}

\url{https://huggingface.co/vialibre}

==> Old/tool.tex <==
\section{Extension of a simple lexical method for bias measurement} \label{sec:tool}

\subsection{Use cases and design goals}

\begin{itemize}
    \item dataset measurement and exploration 
    \item biases exploration in gendered languages
    \item lexical seeds comparison 
    \item 
\end{itemize}

\subsection{Dataset measurement and dataset exploration}


